Provably Robust Score-Based Diffusion Posterior Sampling for Plug-and-Play Image Reconstruction

In a great number of tasks in science and engineering, the goal is to infer an unknown image from a small number of measurements collected from a known forward model describing certain sensing or imaging modality. Due to resource constraints, this task is often extremely ill-posed, which necessitates the adoption of expressive prior information to regularize the solution space. Score-based diffusion models, due to its impressive empirical success, have emerged as an appealing candidate of an expressive prior in image reconstruction. In order to accommodate diverse tasks at once, it is of great interest to develop efficient, consistent and robust algorithms that incorporate unconditional score functions of an image prior distribution in conjunction with flexible choices of forward models. This work develops an algorithmic framework for employing score-based diffusion models as an expressive data prior in general nonlinear inverse problems. Motivated by the plug-and-play framework in the imaging community, we introduce a diffusion plug-and-play method (DPnP) that alternatively calls two samplers, a proximal consistency sampler based solely on the likelihood function of the forward model, and a denoising diffusion sampler based solely on the score functions of the image prior. The key insight is that denoising under white Gaussian noise can be solved rigorously via both stochastic (i.e., DDPM-type) and deterministic (i.e., DDIM-type) samplers using the unconditional score functions. We establish both asymptotic and non-asymptotic performance guarantees of DPnP, and provide numerical experiments to illustrate its promise in solving both linear and nonlinear image reconstruction tasks. To the best of our knowledge, DPnP is the first provably-robust posterior sampling method for nonlinear inverse problems using unconditional diffusion priors.

==> refined_analysis.tex <==


\subsection{Faster convergence for uniquely solvable problems}
Many high-stake inverse problems are supposed to be \emph{uniquely solvable}, i.e., the data $x^\star$ can be uniquely determined by the prior and and measurements. In this part, we will show that faster convergence rate is possible under this assumption. Formally, assume $p^\star$ is supported on some low-dimensional manifold $\cM$, the inverse problem $y=\cA(x)$ is uniquely solvable if
\[
    y = \cA(x), \quad x \in \cM,
\]
has a unique solution $x=x^\star$. This definition works in the noiseless setting. For the noisy setting, the posterior sampling perspective in this paper provides a natural generalization: unique solvability amounts to the property that the posterior distribution $p^\star(x|y)$ concentrates around $x=x^\star$. This idea is made formal in the following definitions.

\begin{definition}[Perturbed posterior distribution]
Let $q_\eta$ be as in \eqref{eqn: q_eta} for all $\eta > 0$, and similarly define
\[
    p^\star_\eta(x) \defeq p^\star(x) * p_{\eta \epsilon}(x) = \frac{1}{(2\pi)^{d/2} \eta^d} \int \rme^{-\frac{1}{2\eta^2} \|x-x'\|^2} p^\star(x') \rmd x', \quad \epsilon \sim \cN(0, I_d).
\]
Define the \emph{perturbed posterior distribution} $\pi^{\mathsf{p}}_{\eta_p, \eta_p}$ with \emph{perturbation level} $(\eta_p, \eta_q)$ as
\[
    \pi^{\mathsf{p}}_{\eta_p, \eta_q}(x) \propto p^\star_{\eta_p}(x) q_{\eta_q}(x).
\]
\end{definition}

\begin{definition}[$\rho$-concentrated distribution]
A probability distribution $p$ is said to be $\rho$-concentrated around some point $x^\star$, where $\rho>0$ is a parameter, if
\[
    \int_{\|x-x^\star\| > r} p(x) \rmd x \le \rme^{-\frac{r^2}{2\rho^2}}, \quad \forall r \ge 10\rho.
\]
\end{definition}

\begin{assumption}[Robust unique solvability]
\label{assum: unique sol}
Assume there exists some constants $\eta_\star, \rho > 0$, such that for all $0 \le \eta_p, \eta_q \le \eta_\star$, the perturbed posterior distribution $\pi^{\mathsf{p}}_{\eta_p, \eta_q}$ is $\rho$-concentrated around $x^\star$.
\end{assumption}

It is easy to verify that $\pi^{\mathsf{p}}_{0, 0}$ is equal to the posterior distribution $p^\star(x|y) \propto p^\star(x) \rme^{\cL(x; y)}$. As such, the perturbed posterior distribution $\pi^{\mathsf{p}}_{\eta_p, \eta_q}$ can be regarded as the true posterior distribution perturbed by noises with level $\eta_p, \eta_q$, and the robust unique solvability assumption imposes that the solution remains close to $x^\star$ (in the sense that the $\|x - x^\star\|$ is small with high probability) as long as the perturbation is small. This assumption is almost sufficient to establish our faster convergence guarantee, but we need one more ingredient to resolve the singularity of distributions.

\begin{definition}[Early-stopping]
For a score function estimation $\hat s$
\end{definition}




\begin{theorem}
There exists some absolute constant $C>0$ such that the following holds.
Under Assumption~\ref{assum: unique sol}, let 
\end{theorem}


